Perils of current DAO governance

DAO Governance is currently broken. We survey the state of the art and find worrying conclusions. Vote buying, vote selling and coercion are easy. The wealthy rule, decentralisation is a myth. Hostile take-overs are incentivised. Ballot secrecy is non-existent or short lived, despite being a human right. Verifiablity is achieved at the expense of privacy. These privacy concerns are highlighted with case study analyses of Vocdoni's governance protocol. This work presents two contributions: firstly a review of current DAO governance protocols, and secondly, an illustration of their vulnerabilities, showcasing the privacy and security threats these entail.

==> Introduction.tex <==
\section{Introduction}
%Greed and money: people want a slice of the pie, especially since they're the ingredients (lambos to the moon). 
%Control: if you have control you decide who gets what. You can bake yourself your own pie.

%Trust (Control implies trust: you 'trust' your cloud provider.
We're observing a paradigm shift towards decentralisation: \sout{Whilst Web 2.0 users can create experiences}, 
Users made Web 2.0, \sout{rewards are reaped by service providers} service providers reaped rewards~\cite{al2012data}, 
\textcolor{red}{What's the motivation for Web3? Sharing the rewards, or concerns over trust?
  I'd bet on rewards, the masses don't understand privacy, it seems twenty-somethings and below are the ones that care.
  (My kid largely objects photos of her face being taken. She doesn't share photos. She complains when others share 
  photos of her. Beyond the kid, I heard a podcast raising surprise that the majority just don't seem to care.)
  I'd suggest dropping the following. It doesn't deserve prime time. (Keep it somewhere! It's a valuable point.)
}
whom users are forced to trust under questionable assurances that said trust is delivered ~\cite{schneble2020google}, ~\cite{berghel2018malice}.
\textcolor{red}{I'm pondering the following, does it deserve prime time. Possibly even less so:
  Facebook vs. Geocities et al. (\url{https://www.google.com/search?q=geocities+ugly&tbm=isch}), 
  Facebook took control from users, managed how content is presented, added UI/UX, ..., 
  the web is better with resource-rich stakeholders taking control.
  READ ON---I'll come back to control in this paragraph, trust too.}
The user has the power to participate, but ultimately it is the main service providers that manage how the content is presented to the user, and which users can upload what ~\cite{nath2014web}. 
\textcolor{red}{(Again, keep these points they're valuable. Perhaps even include them elsewhere, just not here,
  you have a limited window to grab the reader, otherwise they're gone---smoother them with knowledge.}
Web3 \sout{introduces the possibility that} \textcolor{red}{excite me} users actively control services in which they participate ~\cite{sims2019blockchain}. \textcolor{red}{Don't start here---start with getting rich, follow on from the opening sentence, 
  you've intrigued the reader, now explain how they can reap the rewards. Next:} 
\textcolor{magenta}{Returning to the issue of control/trust, is the insight: 
  service providers are utterly untrusted/unable to uphold communities, 
  trust must be distributed amongst netizens who control \emph{their} communities.
  That sounds like a great story.}
\sout{Decentralised decision making---enabled by distributed ledgers---is causing disruption ~\cite{rauchs2018distributed}.}
\textcolor{red}{Possibly editing myself:}
Web3 embraces \sout{distributed ledgers} blockchain to distribute decision making amongst netizens~\cite{rauchs2018distributed}.
\textcolor{red}{Unsure whether \emph{causing disruption} adds value.} 
The participatory nature of these systems is no coincidence, indeed, they were designed to empower the users and circumvent the centralised monopolies. \textcolor{red}{rework the previous two (or three) sentences into one?} 
Whether this actually transpires is hotly contested\sout{, but this}---the revolution's power cannot be denied nor diminished ~\cite{collomb2016blockchain}, ~\cite{maull2017distributed}. \textcolor{red}{avoid the negative; ``regardless, the revolution has power,"
``regardless, a revolution is underway,'' perhaps a quote from a revolutionary will better convey the message.}
 
\textcolor{red}{there's no clear relation between the paragraph above and the one below. Push the above into the body?} \textcolor{blue}{I was trying to set the scene of how DAOs have emerged (ie, built on distributed ledgers) and why they are relevant (ie: they are disruptive because they allow decentralised decision making and users don't have to trust the service providers.}

Decentralised Autonomous Organisations (DAOs)---operation in accordance with rules encoded in smart contracts---are an alternative to centralisation ~\cite{nabben2021DAO}, ~\cite{sims2019blockchain}. 
DAOs follow a `code is law' approach, operating in accordance with rules encoded in smart contracts. These contracts dictate terms and conditions under which certain decisions will be taken. Once the conditions are met, the smart contracts are executed automatically  \cite{smartcontract}, thereby removing the need for a middleman or escrow. Contracts are open source and DAO members can audit  them.

%DAO members must agree on what rules are approved and implemented, and as a consequence, the governance procedure that they use is crucial to ensure fair decision-making. 
Governance is crucial to ensure fair decisions---DAO members must agree on which rules to enact.
Voting schemes are used to aggregate individual views,  providing means of consensus. These have been heavily studied throughout history, and properties to ensure fairness and freedom are established. 

DAOs are relatively new, and arguably esoteric. Voting is neither. 
Disturbingly, DAOs have adopted voting systems that are unfit for purpose---established findings disregarded, warnings and cautionary advice ignored, or slowly and shyly implemented.

\paragraph{Contributions.} First, we collect an updated and expanded summary of the possible attack vectors existing against current voting mechanisms in DAOs. 
Secondly, we propose a series of recommendations on how to mitigate against these attacks and explore the promising proposals that new key players are developing.








==> PathForward.tex <==
\subsection{The Path Forward}
At this point, it is necessary to introduce formalisations of properties that voting systems should satisfy to provide fair and free election outcomes. 
Introduce Ballot Secrecy informally and then formally.
Then Ballot Independence informally and formally.

Proofs in the appendix that one imples the other.

Next, introduce the voting scheme that we propose to solve the DAO failings.

Conclude. 

\noindent Displayed equations are centered and set on a separate
line.
\begin{equation}
x + y = z
\end{equation}


\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}
%
% the environments 'definition', 'lemma', 'proposition', 'corollary',
% 'remark', and 'example' are defined in the LLNCS documentclass as well.
%
\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}

==> oldIntro.tex <==
=======
With the rise of Web3 technologies, the industry has witnessed a paradigm shift towards decentralisation. In Web2, the breakthrough was the ease of consumption for the user, wherein their capabilities extended to allow both read and write actions, as opposed to in Web1, where it was defined by read-only \cite{nath2014web}. The user has the power to participate, but ultimately it is the main service providers that manage how the content is presented to the user, and which users can upload what. Indeed, they own the service, the data that is generated through it, and as a consequence, the financial worth that it bears \cite{al2012data}. This centralisation carries power, and inherently, it demands the users trust said providers. Whether this trust is earned or not has recently been questioned \cite{schneble2020google}, \cite{berghel2018malice}, and users wish to participate not only in the consumption of the services, but also in the decision making that pertains to them \cite{sims2019blockchain}.  
Distributed Ledger Technologies have disrupted the industry by providing a method to enable decentralised decision making \cite{rauchs2018distributed}. The participatory nature of these systems is no coincidence, indeed, they were designed to empower the users and circumvent the centralised monopolies. Whether this actually transpires in practice or not is hotly contested, but the power of this revolution cannot be denied or diminished \cite{collomb2016blockchain}, \cite{maull2017distributed}. 
Exploiting this technology, Decentralised Autonomous Organisations (DAOs) emerged as an alternative approach to centralised organisations \cite{nabben2021DAO}, \cite{sims2019blockchain}. These organisations are run following rules that are encoded in smart contracts. These smart contracts dictate the terms and conditions under which certain decisions will be taken, and are executed automatically once these are met \cite{smartcontract}. They are open source and members of the DAO can audit these smart contracts. DAOs follow a ‘code is law’ approach, where there is no need for a middleman or escrow, as this role is taken over by smart contracts. Participants of the DAO must come to an agreement on what rules are approved and implemented, and as a consequence, the governance procedure that they use is crucial to ensure fair decision-making. 
Voting schemes provide a means to aggregate individual views and return a result. These are the mechanisms that provide solutions to the question of consensus, and have been heavily studied throughout history. While DAOs are relatively new, voting is not. Despite this, DAOs are still using voting mechanisms that are not fit for purpose. Established findings in the academic world of voting have not been taken into consideration when implementing governance solutions, and warnings and cautionary advice by other academics has been ignored, or had shy and slow uptake in the field. In this work, we collect an updated and expanded summary of the possible attack vectors existing against current voting mechanisms in DAOs. Furthemore, we propose a series of recommendations on how to mitigate against these attacks and explore the promising proposals that new key players are developing.
